Example-Based Machine Translation from Text to a Hierarchical Representation of Sign Language

This article presents an original method for Text-to-Sign Translation. It compensates data scarcity using a domain-specific parallel corpus of alignments between text and hierarchical formal descriptions of Sign Language videos in AZee. Based on the detection of similarities present in the source text, the proposed algorithm recursively exploits matches and substitutions of aligned segments to build multiple candidate translations for a novel statement. This helps preserving Sign Language structures as much as possible before falling back on literal translations too quickly, in a generative way. The resulting translations are in the form of AZee expressions, designed to be used as input to avatar synthesis systems. We present a test set tailored to showcase its potential for expressiveness and generation of idiomatic target language, and observed limitations. This work finally opens prospects on how to evaluate translation and linguistic aspects, such as accuracy and grammatical fluency.

==> fig/tab-ex_vaisselle.tex <==
\begin{tabular}{cc}
\toprule
   &
   Files names
   &
   Sentences from the corpus 
    \\ \midrule
    RO1_X0069.Titre1
    &
    Samedi 30 et dimanche 31 mars , de grands chefs ont vendu leur vaisselle en Alsace, à Gerstheim 
    \\ \midrule
    RO1_X0088.Titre2 
    &
    Moins de TVA pour les plus modestes : " Il ne faut pas traiter ça par le mépris ", lance Xavier Bertrand au gouvernement 
    \\ \midrule
    RO1_X0092.Titre1
    &
    Le superéthanol n'est proposé que dans 1 000 stations-service en France, comme ici dans la banlieue de Bordeaux 
    \bottomrule
    
\end{tabular}
